Exqutor: Extended Query Optimizer for Vector-augmented Analytical Queries

Vector similarity search is becoming increasingly important for data science pipelines, particularly in Retrieval-Augmented Generation (RAG), where it enhances large language model inference by enabling efficient retrieval of relevant external knowledge. As RAG expands with table-augmented generation to incorporate structured data, workloads integrating table and vector search are becoming more prevalent. However, efficiently executing such queries remains challenging due to inaccurate cardinality estimation for vector search components, leading to suboptimal query plans. In this paper, we propose Exqutor, an extended query optimizer for vector-augmented analytical queries. Exqutor is a pluggable cardinality estimation framework designed to address this issue, leveraging exact cardinality query optimization techniques to enhance estimation accuracy when vector indexes (e.g., HNSW, IVF) are available. In scenarios lacking these indexes, we employ a sampling-based approach with adaptive sampling size adjustment, dynamically tuning the sample size to balance estimation accuracy and sampling overhead. This allows Exqutor to efficiently approximate vector search cardinalities while minimizing computational costs. We integrate our framework into pgvector, VBASE, and DuckDB, demonstrating performance improvements of up to four orders of magnitude on vector-augmented analytical queries.

==> sections/0-revision.tex <==
\clearpage
% \begin{center}
%     {\large\bfseries A Response Letter}
% \end{center}


\begin{strip}
    \centering
    {\Huge Response to Reviewer Comments\\ 
    Exqutor: Extended Query Optimizer for Vector-augmented Analytical Queries\par}
    % 두 제목 사이에 적절한 간격을 줍니다.
    \vspace{2em} 
\end{strip}

% \title{Response to Reviewer Comments\\Exqutor: Extended Query Optimizer for Vector-augmented Analytical Queries}

% \maketitle

\balance

% \vspace{2em} % 제목과 본문 사이의 간격

% \section*{A Response Letter}

We thank the reviewers for their thoughtful comments and constructive suggestions, which have significantly contributed to improving the quality of our paper. In the revised manuscript, we have addressed all the comments and incorporated corresponding updates throughout the text. Below, we provide detailed responses to each point raised. 

\section*{REVIEWER 1}
\begin{comment}
O1: The core idea of using index-based exact counts or sampling for cardinality estimation is straightforward and well-established in traditional database systems. The paper does not introduce any fundamentally new techniques but rather applies existing methods to the vector search domain. The adaptation to vector data, while practical, does not constitute a significant theoretical or algorithmic contribution.
\end{comment}
\begin{point} {R1.O1}
    The core idea of using index-based exact counts or sampling for cardinality estimation is straightforward and well-established in traditional database systems. The paper does not introduce any fundamentally new techniques but rather applies existing methods to the vector search domain. The adaptation to vector data, while practical, does not constitute a significant theoretical or algorithmic contribution.
\end{point}

\begin{response}
We sincerely thank the reviewer for raising this important point about the novelty of our work. We agree that the individual techniques employed in \sysname, such as index-based exact cardinality estimation and sampling, are well-established in the context of traditional relational databases. Our contribution does not lie in proposing a fundamentally new algorithm, but rather in extending and adapting these techniques to the setting of vector-augmented analytical queries (VAQs) that combine vector search with multi-table joins, beyond the single-table attribute filtering considered in prior work. 

To the best of our knowledge, \sysname is the first work to systematically address query optimization for VAQs involving joins with vector predicates. In addition, both techniques in \sysname are carefully adapted to the characteristics of vector data. For queries with vector indexes, we apply ECQO by visiting only tables with vector embeddings and leveraging lightweight ANN indexes, which keep overhead manageable. Prior work has employed ECQO exclusively in offline settings because its computational overhead made it impractical to use during runtime optimization, for example, it was often applied only to test how cost estimators behave under exact selectivities\cite{ecqo_imma, ecqo_test}. In contrast, \sysname incorporates ECQO into runtime planning by reusing ANN results during execution, showing that with lightweight indexes, ECQO can be incorporated into runtime with manageable overhead. For queries without vector indexes, \sysname employs a sampling-based approach. We acknowledge that sampling as a general technique is well-established in traditional query optimization. However, in the context of high-dimensional vector data, diverse distribution over vector datasets posed unique challenges for similarity search, which was the reason ANN indexes were originally introduced. To address this, \sysname adaptively adjusts the sample size based on cardinality-based Q-Error and introduces a momentum-based update mechanism optimized with respect to cardinality metrics. This design improves robustness to workload shifts, as shown in \autoref{fig:adaptive_sample_size}, where the system converges to different equilibrium sample sizes for different datasets.

% At the same time, we note that while prior work has typically used ECQO techniques in a limited fashion, often for testing purposes or by exploiting only partial scans during optimization \cite{ecqo_imma, ecqo_test}, \sysname executes the entire vector predicate at runtime to obtain exact cardinalities. This provides accurate selectivity information directly to the optimizer, which in turn enables more robust plan choices for VAQs.  

We believe that \sysname establishes a foundation for future research on query optimization strategies tailored to the high-dimensional nature of vector data, not only driving further practical impact but also paving the way for theoretical advances in this space.  
\end{response}

\begin{changes}
% Since ECQO can
% incur substantial computational overhead, Exqutor addresses
% this challenge by visiting only tables with vector embeddings
% and reusing the obtained ANN results during execution. \kp{Please say that we clarified ...}
We have revised the contributions in \autoref{sec:intro} to more clearly articulate the novelty of our work. 
In particular, we emphasize that our contributions include proposing the notion of VAQs, incorporating ECQO into a runtime setting, and enhancing sampling with a momentum-based mechanism.
\end{changes}

% \begin{response}
% We sincerely thank the reviewer for raising this important point about the novelty of our work. We fully agree that the individual techniques employed in \sysname, such as index-based exact cardinality estimation (ECQO) and adaptive sampling, are well-established in the context of traditional relational databases. Our contribution is not in proposing a fundamentally new algorithm, but rather in extending and adapting these techniques to the setting of vector-augmented analytical queries (VAQs) that combine vector search with multi-table joins, beyond the single-table attribute filtering considered in prior work.

% To the best of our knowledge, \sysname is the first framework that systematically addresses query optimization for VAQs involving joins with vector predicates, exposing unique challenges posed by the curse of dimensionality and the lack of accurate selectivity estimates. In this context, our work demonstrates how classical techniques can be effectively repurposed and integrated into generalized vector database systems (pgvector, VBASE, DuckDB) to achieve substantial practical improvements.

% We acknowledge that the current paper does not yet deliver a fundamentally new theoretical or algorithmic breakthrough. Inspired by the reviewer’s comment, we plan to further investigate novel query optimization strategies tailored to the high-dimensional nature of vector data, aiming to contribute not only practical solutions but also theoretical advances in future work.
% \end{response}

% \begin{response}
% We sincerely thank the reviewer for raising this important point about the novelty of our work. We fully agree that the individual techniques employed in \sysname, such as index-based exact cardinality estimation and adaptive sampling, are well-established in the context of traditional relational databases. Our contribution is not in proposing a fundamentally new algorithm, but rather in extending and adapting these techniques to the setting of vector-augmented analytical queries (VAQs) that combine vector search with multi-table joins, beyond the single-table attribute filtering considered in prior work.
% \rs{add why such extension/adaption is challenging/non-trivial and not straightforward, or why a naive extension/application is not sufficient}

% \rs{to the best of our knowledge \sysname is the first work to ...}

% At the same time, we note that while prior work has typically used ECQO techniques in a limited fashion, often for testing purposes or by exploiting only partial scans during optimization \cite{ecqo_imma, ecqo_test}, \sysname executes the entire vector predicate at runtime to obtain exact cardinalities. This provides accurate selectivity information directly to the optimizer, which in turn enables more robust plan choices for VAQs.

% Looking ahead, we plan to further investigate query optimization strategies specifically tailored to the high-dimensional nature of vector data, building on the foundation established by \sysname to pursue both practical enhancements and theoretical advances in future work.
% \rs{maybe modify it to something like this: \sysname establishes a foundation for future research on query optimization strategies specifically tailored to the high-dimensional nature of vector data as well as for practical impact in this space.}
% \end{response}



\begin{comment}
About novelty

\sysname does not constitute a significant theoretical or algorithmic contribution. Instead, \sysname is the first paper that suggest vector query with joins not only attribute filtering. 
지금까지 vector search를 빠르게 하기 위한 ANN index 연구나 filter까지 처리하기 위한 연구는 다수 진행되었다. 이렇게 연구된 인덱스를 RDBMS에 적용하기도 했지만 모두 single table operation에 그쳤기에 \sysname이 multi table operation with vector search의 문제를 보여주는 첫번째 논문으로 curse of dimension을 극복하기 위한 방법으로 ECQO 와 sampling을 활용했다.

본 논문은 기존에 있는 algorithmic mehthod를 활용했지만 추후에는 curse of dimension을 극복할 수 있을만한 theoretical or algorithmic contribution이 있는 query optimization 연구를 진행하겠다.
\end{comment}

\begin{point} {R1.O2}
    The paper frames its work as the "first" to address VAQ optimization, but the techniques employed are incremental. For example, the use of HNSW indexes for exact counts during planning or momentum-based sampling adjustments are logical extensions of existing methods. The absence of a comparative analysis with alternative approaches (e.g., learned estimators or hybrid methods) further limits the perceived novelty.
\end{point}

\begin{response}
In the revised version, we provide additional discussion and include comparisons with learned cardinality estimators such as SelNet \cite{selnet}. Our experimental results show that \sysname consistently achieves better query execution times than learned estimators. We attribute this advantage to its tight integration into the DBMS optimizer, which allows accurate cardinality estimates to be obtained directly within the system during planning.

We also clarify in the discussion section that learned estimators, while effective in certain contexts, often require substantial offline training and external model management, which introduce overhead and complexity. By contrast, the in-system design of \sysname avoids these issues and provides a more reliable and efficient path for VAQ optimization. This addition highlights the practical benefits of tight optimizer integration beyond what can be achieved with external learned models.
\end{response}
% sampling 관련해서는 query time은 안보여주고 q-error만 활용해서 보여주기
% We thank the reviewer for pointing out the importance of comparative analysis with alternative approaches such as learned cardinality estimators. We fully acknowledge that our initial submission did not emphasize these comparisons clearly enough.

% \begin{changes}
%     % discussion에 learned estimator인 selnet과 query time을 비교한 그림을 추가하였다.
% \end{changes}

\begin{changes}
We have added \autoref{fig:selnet} and an accompanying explanation in the discussion section (\autoref{sec:discussion}) to compare \sysname with the learned cardinality estimator SelNet \cite{selnet}. 
% \rs{the limitation of needing external model management, noted above, could be added in the main paper.}
\end{changes}

% \begin{changes}
% We have added a new subsection in the discussion that provides a direct comparison between \sysname and the learned cardinality estimator SelNet. 
% Specifically, we included a new figure (Figure~\ref{fig:selnet}) showing query execution times on the DEEP dataset (SF10), where \sysname consistently outperforms SelNet. 
% We also reported Q-error results, highlighting that \sysname achieves lower estimation error with significantly less overhead. 
% % This addition addresses the reviewer’s request for a stronger baseline comparison with learned approaches.
% \end{changes}

\begin{comment}
compare with selnet - sigmod 2021
learned cardinality estimator과 쿼리 time에서 더 좋은 성능을 보인다. learned cardinality estimator는 model build를 위해 상당한 시간의 offline processing time을 필요로하며 시스템 외부에서 동작하여 추가적인 overhaed가 있다. \sysname은 DBMS opimizer에 plug 되어 하나의 시스템으로 동작하며 index나 sampling 등 overhead를 최소화하면서 optimal query plan을 찾을 수 있도록 만들게 노력하였다.

\end{comment}

\begin{point}{R1.O3}
    Although the experiments show performance improvements, the benchmarks are limited to TPC-H extensions with synthetic vector data. The paper does not sufficiently explore real-world scenarios (e.g., dynamic workloads, skewed distributions) or compare with state-of-the-art baselines beyond default configurations of pgvector/VBASE/DuckDB.
\end{point}

\begin{response}
We agree that demonstrating real-world scenarios in the evaluation is important. 
To clarify this aspect, we revised the paper to explicitly mention that the datasets used in our experiments have diverse distributions~\cite{data-distribution}. 
Specifically, the DEEP dataset follows a normal distribution, while the SIFT dataset has a skewed distribution. 
We further conducted experiments on diverse workloads in \autoref{sec:div_workloads} and incorporated additional comparisons against alternative baseline configurations, as illustrated in \autoref{fig:query_time_selectivity}. 
\end{response}

% \rs{I am not sure what the reviewer meant by 'skewed distribution' in the comment. SIFT has a skewed value distribution, but TPC-H data distribution on the relational side is still fairly uniform. Other variants of TPC-H such as JCC-H or skewed TPC-H have been proposed that have the same schema as TPC-H but add skew.}

\begin{changes}
We added a clarification in the paper (\autoref{sec:eval}) that the datasets used in our evaluation have diverse distributions. 
We also introduced new experiments on diverse workloads with vector indexes in \autoref{sec:div_workloads}, including correlated queries (\autoref{fig:yfcc}), multi-vector queries (\autoref{fig:multi-1-table}, \autoref{fig:multi-2-tables}), and TPC-DS (\autoref{fig:tpc-ds}). 
In addition, we incorporated comparisons against other baseline configurations in \autoref{fig:query_time_selectivity}.
\end{changes}
% \rs{add fig. numbers}

\begin{comment}
% tpc-h 도 더 rich하게 만들었다
% \begin{response}
% To broaden the evaluation beyond TPC-H–style setups, we ran additional experiments on datasets widely used for vector similarity search, covering diverse distributions (e.g., skewed, heavy-tailed, clustered) and a range of embedding dimensions from low to high. We also added TPC-DS–style workloads to increase workload variety, including larger join graphs and multiple vector predicates. Across these settings, \sysname continued to show substantial performance improvements while keeping planning overhead low. We report the detailed results in the revised evaluation section.
% \end{response}

    vector similarity search에 많이 사용되면서 distribution과 dimension이 다양한 데이터셋을 활용해서 실험을 진행하였다. workload를 추가하기 위해 TPC-DS에 관해서도 실험을 추가로 진행하으며 이 경우에도 상당한 성능 향상을 보였다.
% https://arxiv.org/pdf/2503.04422
\end{comment}

\begin{point}{R1.O4}
    The paper positions Exqutor as a groundbreaking solution for VAQs, but the implementation (plugin-style integration with existing systems) suggests modest architectural changes. The discussion overlooks limitations, such as the overhead of index maintenance or the applicability of sampling in high-dimensional spaces, which are critical for practical adoption.
\end{point}

\begin{response}
\sysname is designed as a pluggable framework that can be integrated into existing generalized vector database systems supporting vector search and vector indexes. Because of this design choice, the cost of index maintenance is left to the underlying system’s implementation, and \sysname does not directly manage it. Our intention was to demonstrate that even modest extensions in such systems (e.g., pgvector, VBASE, DuckDB) can bring meaningful benefits through more accurate cardinality estimation.

In the revised paper, we also expand the discussion of other limitations. While the overhead of sampling increases with dimensionality due to the higher cost of distance computations, our evaluation shows that the absolute overhead remains small compared to the performance gains achieved. We also acknowledge that \sysname itself introduces additional planning overhead, and we recognize this as a valid concern. Nonetheless, we consider accurate cardinality estimation to be critical for generating better plans. To balance overhead with estimation accuracy, \sysname employs an adaptive sampling strategy, which dynamically adjusts the sample size to maintain efficiency while still providing reliable selectivity estimates.
\end{response}

\begin{changes}
We added a new limitations subsection (\autoref{sec:limitations}), covering index maintenance costs and sampling overhead in high-dimensional datasets.
\end{changes}

% index 는 underlying system에서 관리한다는 내용을 어디에 넣어야될까
\begin{comment}
O4: The paper positions Exqutor as a groundbreaking solution for VAQs, but the implementation (plugin-style integration with existing systems) suggests modest architectural changes. The discussion overlooks limitations, such as the overhead of index maintenance or the applicability of sampling in high-dimensional spaces, which are critical for practical adoption.
\end{comment}

% By clarifying these aspects, we aim to provide a balanced perspective: \sysname is not a fundamental redesign of query optimization, but a lightweight and practical extension that achieves measurable improvements in real systems.


% 이미 vector search를 지원하고 벡터 인덱스를 활용할 수 있는 database system에 plug 할 수 있으며 index maintenance는 각 시스템에 dependent 하다. sampling overhead가 dimension이 증가하면서 overhaed가 증가하지만 그래도 여전히 gain에 비해서는 굉장히 적은 수치를 보여주고 있다.

% \begin{response}
% We thank the reviewer for pointing out this important issue. \sysname is a pluggable framework that can be integrated into existing generalized vector database systems that already support vector search and vector indexes. This design choice was intentional: our goal was to demonstrate that even with modest extensions, systems such as pgvector, VBASE, and DuckDB can benefit significantly from accurate cardinality estimation.

% Regarding the limitations, we have added clarifications in the revised paper. First, index maintenance overhead indeed depends on the implementation of the underlying system, and \sysname does not directly manage or reduce this cost, since it operates on top of existing vector indexes provided by the DBMS. Second, we acknowledge that sampling overhead grows with dimensionality. However, our evaluation shows that the absolute overhead remains negligible compared to the performance gains, even for high-dimensional datasets.

% By clarifying these aspects, we aim to provide a more balanced view of \sysname: while it does not remove fundamental costs such as index maintenance, it nonetheless offers a lightweight and practical extension that achieves measurable benefits in real-world database systems.
% \end{response}


\begin{comment}
    \begin{response}
\sysname is designed as a pluggable framework that can be integrated into existing generalized vector database systems supporting vector search and vector indexes. Our intention was to demonstrate that even modest extensions in such systems (e.g., pgvector, VBASE, DuckDB) can bring meaningful benefits through more accurate cardinality estimation.   

In the revised paper, we also expand the discussion of limitations. Index maintenance overhead remains dependent on the implementation of the underlying system, and \sysname does not directly manage this cost. We further note that while sampling overhead increases with dimensionality, our evaluation shows that the absolute overhead is small compared to the performance gains observed.
% 논문에 이 내용 몇줄 추가
% overhead에 대한 concern이 있다. agree - 그래서 adaptable하게 sample size를 조절하도록 만들었다. 
% 좀더 claer 하게 overhead가 있다는 거를 인정하도록 작성 - 그래서 이거를 어떻게 조절하려고 했다. 

\end{response}
\end{comment}

\begin{comment}
    We thank the reviewer for pointing out this important issue. We agree that Exqutor should not be seen as a completely new query optimizer architecture, but rather as a pluggable framework that can be integrated into existing systems that already support vector search and vector indexes. This design choice was intentional: our goal was to demonstrate that even with modest extensions, generalized vector DBMSs (e.g., pgvector, VBASE, DuckDB) can benefit significantly from accurate cardinality estimation.

Regarding the limitations, we have added clarifications in the revised paper. First, index maintenance overhead indeed depends on the underlying system’s implementation, and Exqutor itself does not eliminate this cost. Second, we acknowledge that sampling overhead grows with dimensionality. However, our evaluation shows that the absolute overhead remains negligible compared to the performance gains, even for high-dimensional datasets.
\end{comment}



\section*{REVIEWER 2}
\begin{point}{R2.O1}
    O1) The experiments focus mostly on TPC-H-like queries (Q3, Q5, Q8, Q9, etc.) with single vector predicates (Section IV, Figure 4). The lack of experiments on multi-vector queries, mixed workloads, or larger query templates leaves open questions about scalability to more complex workloads.
\end{point}

\begin{response}

\begin{figure}
    \centering
    \includegraphics[width=0.8\linewidth]{figures/vaq_tpc-h_schema.pdf}
    \caption{The TPC-H VAQs schema}
    \label{fig:tpch_schema}
\end{figure}

We thank the reviewer for raising this important concern. In the revised version, we first extended the TPC-H Vector-augmented SQL analytics by incorporating multi-vector queries to evaluate scenarios with multiple vector predicates by adding text and image embeddings in partsupp table and also other image embeddings in part table (\autoref{fig:tpch_schema}). In addition, we added TPC-DS workloads to \benchmarkname for larger query templates and more complex join graphs, the details of which are available at \url{https://gitfront.io/r/bdai-research/68PkKJN7keA4/Exqutor/tree/Vector-augmented_SQL_analytics/tpc-ds/}, to further test scalability under diverse workloads. For VA These additional experiments show that \sysname continues to provide substantial performance improvements even in more complex and realistic conditions.



\end{response}

\begin{changes}
We have extended the evaluation in (\autoref{sec:div_workloads}) by incorporating multi-vector queries into the TPC-H Vector-augmented SQL analytics benchmark (\autoref{fig:multi-1-table}, \autoref{fig:multi-2-tables}) and by adding TPC-DS workloads with larger query templates and more complex join graphs (\autoref{fig:tpc-ds}).
\end{changes}

\begin{comment}
    O1) The experiments focus mostly on TPC-H-like queries (Q3, Q5, Q8, Q9, etc.) with single vector predicates (Section IV, Figure 4). The lack of experiments on multi-vector queries, mixed workloads, or larger query templates leaves open questions about scalability to more complex workloads.
\end{comment}
% \begin{response}
% multi query vector 추가, tpc-ds 에서도 실험해서 다양한 workload, query 를 실험을 했다. 
% \end{response}
\begin{comment}
    We sincerely thank the reviewer for pointing out this important concern. We agree that the initial experiments were focused on TPC-H–like queries with single vector predicates, which limited the generality of our evaluation. In the revised paper, we extend the experiments to include multi-vector queries and mixed workloads, and we also incorporate TPC-DS–style templates with larger join graphs. These additional evaluations demonstrate that Exqutor continues to provide substantial improvements even under more complex workloads, thereby addressing scalability and robustness concerns.
\end{comment}

\begin{point}{R2.O2}
    O2) The experimental baselines are limited to the default query optimizers in pgvector, VBASE, and DuckDB (Section VI-A). The paper does not evaluate Exqutor against state-of-the-art learned or adaptive query optimizers, which could provide stronger evidence of its superiority.
\end{point}


\begin{response}
    In the revised version, we added comparisons with state-of-the-art learned cardinality estimators designed for high-dimensional vector data such as SelNet \cite{selnet}. Our results show that \sysname consistently achieves better query execution times, which we attribute to its tight integration into the DBMS optimizer. By contrast, learned estimators require substantial offline training and external model management, introducing overhead and complexity. We have reflected this discussion in the paper to highlight the practical benefits of \sysname’s in-system design.
\end{response}

\begin{changes}
We have added a comparison with the learned cardinality estimator SelNet \cite{selnet} in the discussion section (\autoref{sec:discussion}), and included a new figure (\autoref{fig:selnet}).
\end{changes}

% \begin{changes}
%     % discussion에 learned estimator인 selnet과 query time을 비교한 그림을 추가하였다.
% \end{changes}

\begin{comment}
    The experimental baselines are limited to the default query optimizers in pgvector, VBASE, and DuckDB (Section VI-A). The paper does not evaluate Exqutor against state-of-the-art learned or adaptive query optimizers, which could provide stronger evidence of its superiority.
\end{comment}

% \begin{response}
% high dimensional data - vector data 를 위한 model을 활용하는 learned cardinality estimator와 비교하였다. 이 방법과 비교했을 때 더 좋은 성능을 보이고 있으며 exqutor는 db system에 더욱 integrate 된다. 
% \end{response}



\section*{REVIEWER 3}
\begin{point}{R3.O1}
    The experiments show that PostgreSQL’s optimizer primarily suffers from overestimating selectivity for vector predicates, raising the question of whether simply lowering the fixed selectivity value in traditional methods could achieve performance comparable to ECQO. It is also unclear whether underestimating the cardinality of embedding filters would conversely lead to worse execution times, which the paper does not analyze. This further suggests that the experimental setting (e.g., always using a threshold that returns 1\% of rows for sampling-based VAQs) might be overly simplified and biased toward ECQO’s strengths.
\end{point}

\begin{response}
We thank the reviewer for this careful observation. We agree that since \benchmarkname employs vector distances with very high selectivity, it is reasonable to question whether simply lowering the fixed selectivity value could be sufficient. To address this, we conducted experiments presented in \autoref{fig:query_time_selectivity}, where we compared query performance at varying selectivity levels. The results show that lowering the fixed selectivity value alone does not consistently yield optimal query plans, what matters is how closely the estimated cardinality aligns with the actual cardinality.
\end{response}

\begin{changes}
We added new experiments in \autoref{fig:query_time_selectivity} that evaluate query performance at varying fixed selectivity levels, and clarified that optimal plans depend on the alignment between estimated and actual cardinalities, rather than simply lowering selectivity values alone.
\end{changes}
% \begin{response}
%     We thank the reviewer for this careful observation. While lowering the fixed selectivity value can sometimes improve performance, it does not generalize well across diverse workloads. In our extended experiments with TPC-DS queries, we observed that such manual adjustment sometimes helped, but in other cases led to severe underestimation, with execution times up to 22{\small$\times$} slower than pgvector and 180{\small$\times$} slower than \sysname when executing queries with HNSW vector index. These results confirm that aligning estimated and true cardinalities is more robust than relying on static heuristics.
% \end{response}




% \begin{response}
% 중요한건 optimizer 가 활용할 수 있는 estimated cardinality 와 true cardinality가 얼마나 비슷하고 이를 통해 최적화된 쿼리를 실행하게 되는지이다. simply lowering the fixed selectivity value하는 건 workload 마다 효과적일 수도, 그렇지 않을 수 있기에 적합하지 않을 수 있다. 실제로 tpc-ds 쿼리에서 lowering the fixed selectivity value 했을 때 기존 시스템 대비 좋은 성능을 보이기도 했지만 일부 쿼리에서는 pgvector 에 비해 22배 느려지고, \sysname 대비 180 느린 성능을 보이기도 하였다. 
% \end{response}

\begin{point}{R3.O2}
    The benchmark is overly simplified, as it only includes a single table with an embedding filter. In such a setting, simply executing that table first naturally leads to better performance. In real-world scenarios, could there be multiple tables containing embedding filters, requiring the optimizer to determine an effective join order? The paper does not explore these more complex cases, which limits the benchmark’s representativeness and the generality of the reported results.
\end{point}
\begin{comment}
    O2. The benchmark is overly simplified, as it only includes a single table with an embedding filter. In such a setting, simply executing that table first naturally leads to better performance. In real-world scenarios, could there be multiple tables containing embedding filters, requiring the optimizer to determine an effective join order? The paper does not explore these more complex cases, which limits the benchmark’s representativeness and the generality of the reported results.
\end{comment}

% \begin{response}
% multiple tables containing embedding filters 에 관련해서도 실험을 진행. 모든 vector range search에 관해서 전부 적용 가능
% \end{response}

\begin{response}
In the revised version, we extended the evaluation to queries where multiple tables contain embedding filters, as illustrated in \autoref{fig:tpch_schema}. These scenarios require the optimizer to determine effective join orders under multiple vector predicates. Our results show that \sysname can be applied to all vector range search nodes in such queries and continues to provide accurate estimates and improved plans. This extension enhances the representativeness of the benchmark.
\end{response}

\begin{changes}
We have extended the evaluation to include queries where multiple tables contain embedding filters, requiring the optimizer to determine effective join orders under multiple vector predicates. 
These results are presented in \autoref{fig:multi-2-tables}.
\end{changes}

\begin{point}{R3.O3}
    The paper does not consider the correlation between embedding attributes and other columns, instead assuming independence, and its benchmark also appears to be constructed under this assumption. This simplification may lead to inaccurate cardinality estimation in scenarios where strong correlations exist, limiting the applicability of the proposed approach in real-world datasets
\end{point}

\begin{response}
To address this point, we conducted additional experiments using the YFCC dataset \cite{yfcc} from the BigANN benchmark \cite{annbenchmark23}, which combines image embeddings with tag attributes. These queries involve both embedding predicates and tag-based filters, thereby introducing correlations between vector and relational attributes. 
Concretely, the dataset consists of a 10M subset of the YFCC 100M corpus with CLIP embeddings, where each image is associated with a bag of tags (e.g., words from the description, camera model, year, and country) drawn from a vocabulary of over 200K possible tags. 
The results show that \sysname remains effective in this setting, since it estimates cardinality at nodes that include both vector search and relational filters. We added this evaluation to the revised paper to demonstrate applicability beyond the independence assumption.
\end{response}

\begin{changes}
We added an evaluation with the YFCC dataset (\autoref{fig:yfcc}) to show query performance under correlations between vector embeddings and tag attributes.
\end{changes}

\begin{comment}
    O3. The paper does not consider the correlation between embedding attributes and other columns, instead assuming independence, and its benchmark also appears to be constructed under this assumption. This simplification may lead to inaccurate cardinality estimation in scenarios where strong correlations exist, limiting the applicability of the proposed approach in real-world datasets

big ann benchmark Filter track에서 활용하는 yfcc 데이터셋을 활용하여 추가 실험을 진행하였다. 이는 image embedding과 관련된 tag 데이터를 포함하며 쿼리에도 임베딩과 tag filtering이 들어간다. Exqutor는 vector range search 뿐만 아니라 다른 filtering 이 포함된 node를 실행하여 cardinality estimation을 진행하기 때문에 이 경우에도 효과적인 성능 향상을 보인다. 

\end{comment}


\begin{table}[t]
\centering
\caption{Comparison of page loads and HNSW index page of pgvector across datasets and scale factors.}
\label{rev:tab:hnsw-pages}
\footnotesize
\begin{tabular}{llrrr}
\toprule
\textbf{Dataset} & \textbf{Metric} & \textbf{SF1} & \textbf{SF10} & \textbf{SF100} \\
\midrule
\multirow{2}{*}{DEEP} 
  & Page loads & 8,204   & 9,390    & 9,785 \\
  & Index pages & 67,792  & 677,766  & 6,777,485 \\
\midrule
\multirow{2}{*}{SIFT} 
  & Page loads & 8,235   & 9,729    & 10,575 \\
  & Index pages & 81,272  & 812,543  & 8,125,935 \\
\midrule
\multirow{2}{*}{SimsearchNet++} 
  & Page loads & 13,146  & 16,410   & 13,120 \\
  & Index pages & 133,373 & 1,333,692 & 13,336,824 \\
\bottomrule
\end{tabular}
\end{table}



\begin{point}{R3.O4}
    The paper claims that PostgreSQL significantly overestimates the cost of ANN index scans due to high space amplification. However, based on their own description (e.g., ANN indexes exceeding base table size), it seems more plausible that the cost model may actually underestimate the real cost, since large index structures and distance computations are not fully modeled. This point requires clarification.
\end{point}

\begin{response}
We clarified this point in the revised paper. While ANN indexes such as HNSW do require substantial storage overhead, their query-time complexity grows approximately as $O(\log \mathit{Card}(T))$~\cite{hnsw}, rather than linearly with the number of indexed vectors. PostgreSQL’s current cost model, which primarily relates index scan cost to index size, therefore tends to overestimate the actual cost of HNSW-based searches. As a result, the optimizer may fail to select an HNSW index scan even in cases where it would be the superior access method.  

To support this, we measured page I/O loads for the same set of query vectors on the DEEP, SIFT, and SimSearchNet++ datasets across scale factors 1, 10, and 100. As shown in \autoref{rev:tab:hnsw-pages}, index sizes grow nearly linearly with dataset scale, but the number of page loads during HNSW index search increases only modestly and in a sublinear fashion.
\end{response}

% \rs{it is not clear to me why accuracy of modeled cost vs actual cost should matter. the role of the cost model is to help choose between alternative plans, so as long as the ranking remains good, it should be fine.}
% due to overestimation, hnsw index scan would not be selected even when hnsw is a better scan method

\begin{changes}
We added a discussion of the computational complexity of HNSW search and clarified in limitations (\autoref{sec:limitations}) that the current cost model does not adequately capture these characteristics, which can result in suboptimal query plan choices.
\end{changes}

\begin{comment}
    O4. The paper claims that PostgreSQL significantly overestimates the cost of ANN index scans due to high space amplification. However, based on their own description (e.g., ANN indexes exceeding base table size), it seems more plausible that the cost model may actually underestimate the real cost, since large index structures and distance computations are not fully modeled. This point requires clarification.

\begin{response}
hnsw 는 log(|D|) 의 query time complexity를 보이며 이로 인해 |D|가 충분히 큰 상황이라면 |D|가 커진다고 해서 query time이 크게 증가하지 않는다. 실제로 hnsw 중 발생하는 page io 를 측정해봐도 linear하게 증가하지 않는 것을 확인할 수 있었다. 

% hnsw 는 high space amplification 문제가 있지만 query time 은 log(|D|) complexity를 갖고 있음 
\end{response}
\end{comment}



\begin{point}{R3.O5}
    The Data Scalability section refers to Q20, but the corresponding figure does not include Q20 (may be Q3?). This inconsistency makes it unclear whether the reported observations (e.g., performance trends) are based on Q20 or Q3.
\end{point}
\begin{comment}
    
O5. The Data Scalability section refers to Q20, but the corresponding figure does not include Q20 (may be Q3?). This inconsistency makes it unclear whether the reported observations (e.g., performance trends) are based on Q20 or Q3.
\end{comment}
\begin{response}
We thank the reviewer for catching this mistake. The issue was in the legend of the corresponding figure, where the label was incorrectly written as Q10. We have corrected this in the revision so that the legend now properly refers to Q20.
\end{response}

\begin{changes}
    We corrected all the errors we found, which are highlighted in the paper.
\end{changes}

\section*{REVIEWER 4}
\begin{point}{R4.O1}
     Exqutor seems to be a net improvement in terms of query optimization compared to the baselines. In the same vein as Figure 7, it would be interesting to see what are the most common query plan improvements that Exqutor brings. For instance, are the execution improvement more due to join reorderings, predicate pushdown, or use of indices instead of full scans? Are the types of improvement consistent over different workloads?
\end{point}
\begin{comment}
    O1. Exqutor seems to be a net improvement in terms of query optimization compared to the baselines. In the same vein as Figure 7, it would be interesting to see what are the most common query plan improvements that Exqutor brings. For instance, are the execution improvement more due to join reorderings, predicate pushdown, or use of indices instead of full scans? Are the types of improvement consistent over different workloads?
\end{comment}

\begin{comment}
    
\end{comment}

\begin{response}
We thank the reviewer for this insightful question. We believe the performance improvements observed with \sysname result from a combination of factors. At the core of these improvements is the ability to provide accurate cardinality estimation, which directly drives better join reordering decisions. Once the optimizer has a more accurate view of join selectivities, it is able to place the most selective joins earlier in the plan. This reordering often enables the use of index scans instead of full scans and, in some cases, leads to the selection of more efficient join methods. Together, these adjustments substantially improve execution performance.  

To examine whether such improvements are consistent across different workloads, we also conducted experiments with TPC-DS queries. The results show that similar types of plan improvements appear in this workload as well, confirming that the benefits of \sysname are not limited to a single benchmark but extend to more complex query templates.

Most query execution improvements are driven by three effects: join ordering, join method changes, and scan method changes. The most common pattern is a transition from hash joins to nested-loop joins and from full scans to index-based access. In some cases, we also observe that bitmap-index scans are replaced by index scans (e.g., Query 5 in TPC-H). Additional examples of such query plan improvements can be found in the supplementary figures on the link (\url{https://gitfront.io/r/bdai-research/68PkKJN7keA4/Exqutor/tree/query_plans/}).


% github에 appendix 추가 tpc-h 쿼리에 대해서 
% 쿼리별로 query plan 비교 그려서 넣어두기 - 성능 향상 요소 정리해서 넣어두기
% 스키마는 github에 넣어서 그림을 찾아볼 수 있다.
\end{response}

\begin{changes} We revised the paper to add a summary that explicitly addresses this point (\autoref{sec: querytime}), describing the most common improvements from \sysname. These improvements mainly arise from join reordering, changes in join methods (e.g., replacing hash joins with nested-loop joins), and transitions in scan methods (from full or bitmap-index scans to index scans). We also note that these patterns appear across workloads such as TPC-DS, demonstrating the general benefits of \sysname. For further illustration, we added references to supplementary figures in Footnote 3 that illustrate additional query execution improvements.  
\end{changes}

% R1.Availabilty
% 코드 script로 만들어서 결과 받을 수 있게 해놨다고 작성

\bigskip \noindent \textbf{R4.Availability:} We thank the reviewer for the helpful suggestions. We have updated the repository to include scripts that automatically download the required files and generate the experimental results reported in the paper.

==> sections/10-ai_acknowledgement.tex <==
\section*{AI-Generated Content Acknowledgement}
We used ChatGPT to assist with minor language-related tasks during the preparation of this manuscript, including English proofreading, grammar checking, and phrasing refinement. All AI-assisted outputs were carefully reviewed, verified, and edited by the authors to ensure accuracy and correctness. The conceptual contributions, technical ideas, analyses, and results presented in this paper are entirely the work of the authors.

==> sections/99-implementation.tex <==
\section{IMPLEMENTATION}



% We have implemented our optimization techniques in \texttt{pgvector}, an extension for PostgreSQL, and \texttt{duckdb\_vss}, an extension for DuckDB, both of which are widely-used open-source generalized vector databases. These implementations extend the capabilities of the query optimizer to efficiently handle vector similarity queries with accurate cardinality estimation.
% , as illustrated in Figure 4.

\sysname is designed to integrate seamlessly into the query optimizers of generalized vector databases, supporting accurate cardinality estimation for vector similarity queries, while it is adaptable to various systems. The framework extends the existing optimizer with a dedicated cardinality estimator, enabling precise estimation. %during the planning phase.

We implemented \sysname into two generalized vector database systems, \texttt{pgvector} for PostgreSQL and \texttt{duckdb\_vss} for DuckDB. By integrating our implementation into each extension, we enabled the database query optimizers to leverage cardinality estimation techniques for generating optimized query plans.

For a given query, the optimizer first checks if a vector distance search is present. If so, the cardinality is estimated by the following prioritized steps:

\mypar{Index-based cardinality estimation} We integrated index-based cardinality estimation into the query optimizer to take advantage of vector indexes (e.g., HNSW or IVF) for efficient cardinality estimation during the planning phase. When the vector index exists, by executing a lightweight vector range search with the index, the optimizer retrieves the actual cardinality of the data points within the specified range. This precise estimate is then passed to the planner, enabling the construction of an optimal query execution plan that minimizes intermediate results and selects the most efficient query plan. To avoid executing the same ANN index search twice, we saved the search results in the planning phase, so that we can get and utilize them in the main query execution step. This allowed us to reduce the AQP overhead and improve performance further.

% \mypar{Model-Based Cardinality Estimation} To handle scenarios where vector indexes are unavailable, we extended the query optimizer to incorporate model-based cardinality estimation. 
% To efficiently train the model, we employed optimized product quantization (OPQ) \cite{OPQ} to construct a compact codebook that represents the dataset. Then, we concatenated the codewords of each subvector to get a well-constructed codebook and used them to train the model for similarity cardinality estimation. This codebook enables the selection of a smaller, representative subset of the data for training, significantly reducing both training time and computational overhead while maintaining high accuracy. 

% To utilize the trained model, \sysname checks that the cardinality estimation model exists and loads the model using the python API if vector indexes don't exist. During the planning phase, \sysname parses the given embedding and distance threshold and passes them to the model to predict the cardinality within the given threshold. Then, the planner gets the estimated cardinality for vector range search and passes the optimized query plan to the executor.

% During query planning, the estimated cardinality from the model is passed to the planner, ensuring that join ordering and query execution plans are optimized for performance. 
% This method is particularly effective for complex workloads where index-based estimation is not feasible.

% \mypar{Model-Based Cardinality Estimation} We enhanced the query optimizer by incorporating model-based cardinality estimation. When a trained cardinality estimation model is accessible, the optimizer uses it to predict the expected cardinality for a given vector range search. The model takes query parameters, such as the vector point and range threshold, as input and produces an estimated cardinality based on learned patterns from the data distribution.

% To ensure that the training process remains computationally efficient while maintaining accuracy, we leveraged product quantization (PQ) to create a codebook representing the dataset. This codebook was then used to select a smaller but representative subset of training data. By training the model on this reduced dataset, we significantly minimized training time without compromising the accuracy of the cardinality estimates.
% This approach is particularly useful when vector indexes are not present or when queries require deeper insights into data distribution. Incorporating model-based estimates into the query planner ensures efficient execution plans while reducing reliance on index-specific operations. By using the PQ-based training data, we achieved high accuracy with minimal training overhead, improving both query planning and execution performance.

\mypar{Sampling-based cardinality estimation} For scenarios where neither vector indexes nor trained models are available, we implemented sampling-based cardinality estimation as a fallback method. 
This method estimates cardinality by analyzing a sampled subset of the data during the planning phase. We calculate the sampling size using the \textit{sample size formula} described in \autoref{sec:sampling}. Due to the limitation of \textit{duckdb}, sampling based method was not implemented in \textit{duckdb}.


% By dynamically selecting the sample size based on query complexity and dataset characteristics, the system balances the trade-off between estimation accuracy and computational overhead.

% system archi 느낌으로, 기존에 있는 시스템에 어떻게 플러거블하게 들어가는지 잘 나올 수 있게
% 시스템 아키 피겨 많이 살펴보기
% extension으로 들어가는 내용의 논문 figure 참고
% QOaas - vision paper

% \begin{figure} [tb!]
%     \centering
%     \includegraphics[width=1\linewidth]{figures/Architecture.png}
%     \caption{A pluggable system with \sysname}
%     \label{fig:architecture}
%     \vspace{-20pt}
% \end{figure}


\begin{figure} [tb!]
    \centering
    \includegraphics[width=1\linewidth]{figures/exqutor3.png}
    \caption{Pluggable Framework Exqutor}
    \label{fig:exqutor3}
    \vspace{-20pt}
\end{figure}


% While sampling is inherently less precise than index-based or model-based methods, it provides a practical solution when no pre-computed resources are available. The estimated cardinality is used to refine the query plan, minimizing unnecessary intermediate results. However, the effectiveness of sampling decreases for highly skewed data distributions or queries involving complex subqueries.

\mypar{Integration into query optimization pipeline} The cardinality estimation methods are integrated into the query optimization pipeline as a modular component.
% , as shown in Figure~\ref{fig:architecture}. During query planning, 
The query optimizer dynamically selects the most appropriate estimation method based on the availability of resources (indexes, models, or sampling capabilities). The cardinality estimates are then used to refine join orders, prune unnecessary query paths, and optimize execution plans for both vector similarity queries and hybrid workloads combining relational and vector operations.

\mypar{Integration and pluggability} The cardinality estimation framework was designed to be modular and pluggable, allowing its methods to be seamlessly integrated into various generalized vector database systems. This design enabled us to apply the same approach used in \texttt{pgvector} to \texttt{duckdb\_vss}, ensuring consistency and adaptability across platforms. 
In \texttt{duckdb\_vss}, we extended the existing optimizer, which originally supported only HNSW indexes for single-table Top-K queries, to handle range-based vector similarity queries and join operations involving vector distances. While index-based and model-based cardinality estimation methods were implemented to provide precise and efficient cardinality estimates during query planning, sampling-based estimation was not included due to system-specific limitations.

Our goal is to demonstrate that the framework can be effectively implemented in other database systems and to facilitate its adoption in additional generalized vector databases. The modular and pluggable nature of the framework ensures that its core components can be adapted to diverse architectures and query optimization pipelines, enabling standardized improvements in query planning for vector similarity queries across platforms.




% We implemented a modular cardinality estimation framework in two generalized vector database systems, \texttt{pgvector} for PostgreSQL and \texttt{duckdb\_vss} for DuckDB. This framework integrates seamlessly into their query optimization pipelines, enabling accurate cardinality estimation for vector similarity queries.

% \paragraph{Integration into PostgreSQL and DuckDB.} 
% In \texttt{pgvector}, the framework was fully integrated into the planning phase to support index-based, model-based, and sampling-based estimation methods. The optimizer dynamically selects the appropriate method based on resource availability (e.g., vector indexes or trained models). In \texttt{duckdb\_vss}, the optimizer was extended to support range-based vector similarity queries and join operations. Due to system-specific constraints, sampling-based estimation was not included. Instead, we focused on index-based and model-based methods to enhance query planning.

% \paragraph{Pluggability.}
% The framework was designed to be modular, allowing its core components to be adapted to diverse architectures. This approach facilitated the reuse of the same techniques across \texttt{pgvector} and \texttt{duckdb\_vss}, demonstrating its adaptability to different systems.

% \paragraph{Challenges and Adaptations.}
% The implementation required modifications to support vector similarity search within the relational optimization frameworks of PostgreSQL and DuckDB. For example, integrating model-based estimation involved handling the prediction overhead during planning. The rule-based decision process was incorporated to ensure prediction costs were justified relative to query complexity.

% By implementing this framework, we demonstrated its feasibility and scalability for improving query optimization in generalized vector databases. The modular design ensures its applicability to other systems, paving the way for standardized support for vector similarity queries in database environments.
